Renyi Differential Privacy of the Subsampled Shuffle Model in Distributed Learning

We study privacy in a distributed learning framework, where clients collaboratively build a learning model iteratively through interactions with a server from whom we need privacy. Motivated by stochastic optimization and the federated learning (FL) paradigm, we focus on the case where a small fraction of data samples are randomly sub-sampled in each round to participate in the learning process, which also enables privacy amplification. To obtain even stronger local privacy guarantees, we study this in the shuffle privacy model, where each client randomizes its response using a local differentially private (LDP) mechanism and the server only receives a random permutation (shuffle) of the clients' responses without their association to each client. The principal result of this paper is a privacy-optimization performance trade-off for discrete randomization mechanisms in this sub-sampled shuffle privacy model. This is enabled through a new theoretical technique to analyze the Renyi Differential Privacy (RDP) of the sub-sampled shuffle model. We numerically demonstrate that, for important regimes, with composition our bound yields significant improvement in privacy guarantee over the state-of-the-art approximate Differential Privacy (DP) guarantee (with strong composition) for sub-sampled shuffled models. We also demonstrate numerically significant improvement in privacy-learning performance operating point using real data sets.

==> app_ternary_special_case.tex <==
\subsection{Proof of Theorem~\ref{thm:ternary_special_case}: Ternary $|\chi|^{\alpha}$-DP of the Special Case}\label{sec:app_ternary_special_case} 

First, we present the following lemma which is crucial in our proof.

\begin{lemma}\label{lemm:traingle_inequality} 
Let $X$ and $Y$ be two random variables. For all $j\geq 1$, we have
\begin{equation}
\mathbb{E}\left[\left|X+Y\right|^{j}\right]\leq 2^{j-1}\left(\mathbb{E}\left[\left|X\right|^{j}\right]+\mathbb{E}\left[\left|Y\right|^{j}\right]\right)
\end{equation}
\end{lemma}
\begin{proof}
The proof is simple from the convexity of the functions $f(x)=x^{j}$ and $g(x)=|x|$. 
\begin{equation}
\begin{aligned}
\mathbb{E}\left[\left|X+Y\right|^{j}\right]&=2^{j} \mathbb{E}\left[\left|\frac{1}{2} X+\frac{1}{2} Y\right|^{j}\right]\\
&\leq 2^{j}\mathbb{E}\left[\left(\frac{1}{2}\left|X\right|+\frac{1}{2}\left|Y\right|\right)^{j}\right]\\
&\leq 2^{j}\mathbb{E}\left[\frac{1}{2}\left|X\right|^{j}+\frac{1}{2}\left|Y\right|^{j}\right]\\
&=2^{j-1}\left(\mathbb{E}\left[\left|X\right|^{j}\right]+\mathbb{E}\left[\left|Y\right|^{j}\right]\right),
\end{aligned}
\end{equation}
where the first inequality is obtained from the convexity of the function $g(x)=|x|$ on $\mathbb{R}$ and the second inequality is obtained from the convexity of the function $f(x)=x^{j}$ on $\mathbb{R}^{+}$ for all $j\geq 1$. This completes the proof.
\end{proof}

Now, we are ready to prove Theorem~\ref{thm:ternary_special_case}. From Lemma~\ref{lemm:traingle_inequality}, we get the following corollary.
\begin{corollary}\label{cor:triange_inequality} 
Fix an arbitrary $m\in\bbN$ and consider any three mutually neighboring datasets $\calD_{m},\ \calD'_{m},\ \calD^{''}_{m}$, where $\calD_m=(d,\hdots,d)\in\calX^m$, $\calD'_m=(d,\hdots,d,d')\in\calX^m$ and $\calD^{''}_m=(d,\hdots,d,d^{''})\in\calX^m$. The ternary $|\chi|^{\alpha}$-DP is bounded by
\begin{align*}
&\mathbb{E}_{\bh\sim\calM_{sh}(\calD_m)}\left[\left|\frac{\calM_{sh}(\calD^{'}_m)(\bh)-\calM_{sh}(\calD^{''}_m)(\bh)}{\calM_{sh}(\calD_m)(\bh)}\right|^{\alpha}\right] \\
&\quad\leq 2^{\alpha-1}\left( \mathbb{E}_{\bh\sim\calM_{sh}(\calD_m)}\left[\left|\frac{\calM_{sh}(\calD^{'}_m)(\bh)}{\calM_{sh}(\calD_m)(\bh)}-1\right|^{\alpha}\right]+\mathbb{E}_{\bh\sim\calM_{sh}(\calD_m)}\left[\left|\frac{\calM_{sh}(\calD^{''}_m)(\bh)}{\calM_{sh}(\calD_m)(\bh)}-1\right|^{\alpha}\right]\right).
\end{align*}
\end{corollary}
\begin{proof}
By taking $X=\(\frac{\calM_{sh}(\calD^{'}_m)(\bh)}{\calM_{sh}(\calD_m)(\bh)}-1\)$ and $Y=-\(\frac{\calM_{sh}(\calD^{''}_m)(\bh)}{\calM_{sh}(\calD_m)(\bh)}-1\)$ and applying Lemma~\ref{lemm:traingle_inequality} gives Corollary~\ref{cor:triange_inequality}.
\end{proof}
\begin{remark}
The proof of Corollary~\ref{cor:triange_inequality} does not exploit the fact that $\calD_m,\calD_m',\calD_m^{''}$ are special triple of neighboring datasets such that $(\calD_m,\calD_m',\calD_m^{''})\in\calD_{\same}^m$. In fact, Corollary~\ref{cor:triange_inequality} holds for 
\end{remark}
Hence, from Lemma~\ref{lemm:T_same_Bound} below and Corollary~\ref{cor:triange_inequality}, we get that 
\begin{equation}
\begin{aligned}
\mathbb{E}_{\calM_{sh}(\calD_m)(\bh)}&\left[\left|\frac{\calM_{sh}(\calD^{'}_m)(\bh)-\calM_{sh}(\calD^{''}_m)(\bh)}{\calM_{sh}(\calD_m)(\bh)}\right|^{\alpha}\right]\leq
&\left\{\begin{array}{ll}
4\frac{\left(e^{\epsilon_0}-1\right)^2}{me^{\epsilon_0}}& \text{if\ } \alpha=2\\
\alpha\Gamma\left(\alpha/2\right)\left(\frac{2\left(e^{2\epsilon_0}-1\right)^2}{me^{2\epsilon_0}}\right)^{\alpha/2}& \text{otherwise} 
\end{array}
\right.
\end{aligned}
\end{equation}
This completes the proof of Theorem~\ref{thm:ternary_special_case}. 



\begin{lemma}\label{lemm:T_same_Bound} 
For any pair of neighboring datasets $\calD_{m},\ \calD'_{m}$, where $\calD_m=(d,\hdots,d)\in\calX^m$, $\calD'_m=(d,\hdots,d,d')\in\calX^m$, we have
\begin{equation}
\begin{aligned}
\mathbb{E}_{\calM_{sh}(\calD_m)(\bh)}&\left[\left|\frac{\calM_{sh}(\calD^{'}_m)(\bh)}{\calM_{sh}(\calD_m)(\bh)}-1\right|^{\alpha}\right]\leq \\
&\left\{\begin{array}{ll}
\frac{\left(e^{\epsilon_0}-1\right)^2}{me^{\epsilon_0}}& \text{if\ } \alpha=2\\
\alpha\Gamma\left(\alpha/2\right)\left(\frac{\left(e^{2\epsilon_0}-1\right)^2}{2me^{2\epsilon_0}}\right)^{\alpha/2}& \text{otherwise} 
\end{array}
\right.
\end{aligned}
\end{equation}
\end{lemma}
\begin{proof}
Consider any pair of neighboring datasets $\calD_{m},\ \calD'_{m}$, where $\calD_m=(d,\hdots,d)\in\calX^m$, $\calD'_m=(d,\hdots,d,d')\in\calX^m$. Let $\bp=(p_1,\ldots,p_B)$ and $\bp'=(p'_1,\ldots,p'_B)$ be the probability distributions of the discrete $\eps_0$-LDP mechanism $\calR:\calX\to\calY=[B]$ when its inputs are $d$ and $d'$ respectively, where $p_j=\Pr[\calR(d)=j]$ and $p_j'=\Pr[\calR(d')=j]$ for all $j\in[B]$. Since $\calR$ is $\eps_0$-LDP, we have 
\begin{equation}\label{LDP_constraints}
\begin{aligned}
e^{-\eps_0}\leq \frac{p_j}{p'_j}\leq e^{\eps_0},\qquad \forall j\in[B].
\end{aligned}
\end{equation}
Since $\calM_{sh}$ is a shuffled mechanism, it induces a distribution on $\calA_B^m$ for any input dataset. So, for any $\bh\in\calA_B^m$, $\calM_{sh}(\calD_m)(\bh)$ and $\calM_{sh}(\calD'_m)(\bh)$ are equal to the probabilities of seeing $\bh$ when the inputs to $\calM_{sh}$ are $\calD_m$ and $\calD'_m$, respectively. Thus, for a given histogram $\bh=(h_1,\hdots,h_B)\in\calA^m_B$ with $m$ elements and $B$ bins, we have
\begin{align}
\calM_{sh}(\calD_m)\left(\bh\right)&=\textsl{MN}\left(m,\bp,\bh\right)={m \choose \bh}  \prod_{j=1}^{B} p_j^{h_j} \label{defn-mu_0},\\
\calM_{sh}(\calD'_m)(\bh)&=\sum_{j=1}^{B} p'_j\textsl{MN}\left(m-1,\bp,\tbh_j\right), \label{defn-mu_1}
\end{align}
where $\textsl{MN}\left(m,\bp,\bh\right)$ denotes the Multinomial distribution with ${m \choose \bh}=\frac{m!}{h_1!\cdots h_B!}$.

Let $X:\calA_B^m\to\bbR$ be a random variable associated with the distribution $\calM(\calD_m)$ on $\calA_B^m$, and for any $\bh\in\calA_B^{m}$, define $X(\bh):=m\left(\frac{\calM(\calD'_m)(\bh)}{\calM(\calD_m)(\bh)}-1\right)$. Thus, we get that $\mathbb{E}\left[\left|\frac{\calM_{sh}(\calD^{'}_m)(\bh)}{\calM_{sh}(\calD_m)(\bh)}-1\right|^{\alpha}\right]=\frac{1}{m^{\alpha}}\mathbb{E}\left[|X|^{\alpha}\right]$. From Lemma~\cite[Lemmas~$6,7$]{girgis2021renyi}, we get that
\begin{equation}
\frac{1}{m^{\alpha}}\mathbb{E}\left[|X|^{\alpha}\right]\leq \left\{\begin{array}{ll}
\frac{\left(e^{\epsilon_0}-1\right)^2}{me^{\epsilon_0}}& \text{if\ } \alpha=2, \\
\alpha\Gamma\left(\alpha/2\right)\left(\frac{\left(e^{2\epsilon_0}-1\right)^2}{2me^{2\epsilon_0}}\right)^{\alpha/2}& \text{otherwise}. 
\end{array}
\right.
\end{equation}
This completes the proof of Lemma~\ref{lemm:T_same_Bound}.
\end{proof}

\subsection{Completing the Proof of Theorem~\ref{thm:ternary_DP_shuffle}}\label{subsec_app:completeting-proof}
For simplicity of notation, for any $m\in\{0,1,\hdots,n-1\}$, define 
\begin{align*}
q_m &:= \binom{k-1}{m} q^m(1-q)^{k-m-1} \\
E_m &:= \mathbb{E}_{\bh\sim\calM_{sh}(\calD_{m+1}^{''(k)})}\left[\left|\frac{\calM_{sh}(\calD_{m+1}^{(k)})(\bh)-\calM_{sh}(\calD_{m+1}^{'(k)})(\bh)}{\calM_{sh}(\calD_{m+1}^{''(k)})(\bh)}\right|^{\alpha}\right].
\end{align*} 
First we show an important property of $E_m$ that we will use in the proof.
\begin{lemma}\label{lem:E_m-decreasing}
$E_m$ is a non-increasing function of $m$, i.e., 
\begin{align}
&\mathbb{E}_{\bh\sim\calM_{sh}(\calD_{m+1}^{''(k)})}\left[\left|\frac{\calM_{sh}(\calD_{m+1}^{(k)})(\bh)-\calM_{sh}(\calD_{m+1}^{''(k)})(\bh)}{\calM_{sh}(\calD_{m+1}^{''(k)})(\bh)}\right|^{\alpha}\right] \notag \\
&\hspace{4cm}\leq \mathbb{E}_{\bh\sim\calM_{sh}(\calD_{m}^{''(k)})}\left[\left|\frac{\calM_{sh}(\calD_{m}^{(k)})(\bh)-\calM_{sh}(\calD_{m}^{'(k)})(\bh)}{\calM_{sh}(\calD_{m}^{''(k)})(\bh)}\right|^{\alpha}\right],\label{eq:E_m-decreasing}
\end{align}
where, for any $l\in\{m,m+1\}$, $\calD_{l}^{(k)}=(d^{''}_k,\ldots,d^{''}_k,d_{k})$, $\calD_{l}^{'(k)}=(d^{''}_k,\ldots,d^{''}_k,d^{'}_{k})$, and  $\calD_{l}^{''(k)}=(d^{''}_k,\ldots,d^{''}_k,d^{''}_k)$, each having $l$ elements.
\end{lemma}
\begin{proof}
Lemma~\ref{lem:E_m-decreasing} follows from Lemma~\ref{lem:cvx_tdp} in a straightforward manner.
\end{proof}
Thus, we get
\begin{align}
\mathbb{E}_{\bh\sim\calM_{sh}(\calD^{''})}\left[\left|\frac{\calM_{sh}(\calD)(\bh)-\calM_{sh}(\calD')(\bh)}{\calM(\calD^{''})(\bh)}\right|^{\alpha}\right]&\leq \sum_{m=0}^{k-1}q_mE_m \notag \\ &=\sum_{m<\floor{(1-\gamma)q(k-1)}} q_m E_m+ \sum_{m\geq\floor{(1-\gamma)q(k-1)}} q_m E_m\notag \\
&\stackrel{\text{(a)}}{\leq} E_{0}\sum_{m<\floor{(1-\gamma)q(k-1)}}q_m+\sum_{m\geq\floor{(1-\gamma)q(k-1)}} q_m E_m \notag \\
&\stackrel{\text{(b)}}{\leq}  E_{0}e^{-\frac{q(k-1)\gamma^2}{2}}+\sum_{m\geq\floor{(1-\gamma)q(k-1)}} q_m E_m \notag \\
&\stackrel{\text{(c)}}{\leq} e^{\epsilon_0\alpha}e^{-\frac{q(k-1)\gamma^2}{2}}+\sum_{m\geq\floor{(1-\gamma)q(k-1)}} q_m E_m \notag \\
&\stackrel{\text{(d)}}{\leq} (e^{\epsilon_0}-e^{-\epsilon_0})^{\alpha}e^{-\frac{q(k-1)\gamma^2}{2}}+ E_{(1-\gamma)q(k-1)}. \label{proof_main-result_interim2}
\end{align}
Here, steps (a) and (d) follow from the fact that $E_m$ is a non-increasing function of $m$ (see Lemma~\ref{lem:E_m-decreasing}). Step (b) follows from the Chernoff bound. In step (c), we used that $\calM_{sh}(d_k)=\calR(d_k)$, $\calM_{sh}(d'_k)=\calR(d'_k)$, and $\calM_{sh}(d^{''}_k)=\calR(d^{''}_k)$ which together imply that $E_0=(e^{\epsilon_0}-e^{-\epsilon_0})^{\alpha}$, where the inequality follows because $\calR$ is an $\eps_0$-LDP mechanism. By choosing $\gamma=0.5$ completes the proof of Theorem~\ref{thm:ternary_DP_shuffle}.





==> problem_formulation.tex <==
\section{Problem Formulation}\label{subsec:prob-form} \label{sec:prob-form}


Let $\calD=\left(d_1,\ldots,d_n\right)$ be a dataset consisting of $n$ data points, where $d_i$ is a data point at the $i$'th client that takes values from a set $\calX$. Let $\calR:\calX\to\calY$ be a local randomizer that satisfies the following two properties:
\begin{enumerate}
\item $\calR$ is an $\epsilon_0$-LDP mechanism (see Definition~\ref{defn:LDPdef}). 
\item  The range of $\calR$ is a discrete set, i.e., the output of $\calR$ takes values in a discrete set $\left[B\right]=\left\{1,\ldots,B\right\}$ for some $B\in\mathbb{N}:=\{1,2,3,\hdots\}$. Here, $[B]$ could be the whole of $\mathbb{N}$.
\end{enumerate}

First, we sub-sample without replacement $k\leq n$ clients of the $n$ clients, where $\gamma=\frac{k}{n}$ denotes the sampling parameter. Each client $i$ out of the $k$ clients applies $\calR$ on $d_i$ (each client uses independent randomness for computing $\calR(d_i)$) and sends $\calR(d_i)$ to the shuffler, who shuffles the received $k$ inputs and outputs the result; see Figure~\ref{fig:setup-figure}. To formalize this, let $\calH_k:\calY^k\to\calY^k$ denote the shuffling operation that takes $k$ inputs and outputs their uniformly random permutation. Let $\samp_{k}^{n}:\calX^{n}\to\calX^{k}$ denote the sampling operation for choosing a random subset of $k$ elements from a set of $n$ elements. We define the sampling-shuffling mechanism as
\begin{equation}\label{shuffle-mech}
\calM\left(\calD\right) := \calH_{k}\circ \samp_{k}^{n}\left(\calR\left(d_1\right),\ldots,\calR\left(d_n\right)\right).
\end{equation}
Our goal is to characterize the Renyi differential privacy of $\calM$. 

Since the output of $\calM$ is a random permutation of the $k$ outputs of $\calR$, the server cannot associate the $k$ messages to the clients; and the only information it can use from the messages is the histogram, i.e., the number of messages that give any particular output in $[B]$. We define a set $\calA_{B}^{k}$ as follows
\begin{equation}\label{histogram-set}
\calA_B^{k}=\bigg\lbrace \bh=\left(h_1,\ldots,h_B\right):\sum_{j=1}^{B}h_j=k\bigg\rbrace,
\end{equation}
to denote the set of all possible histograms of the output of the shuffler with $k$ inputs. Therefore, we can assume, without loss of generality (w.l.o.g.), that the output of $\calM$ is a distribution over $\calA_B^{k}$ for input dataset $\calD$ of $n$ data points.


\begin{figure}[t]
\centering \includegraphics[scale=0.35]{setup-figure.pdf}
\caption{In the shuffled model, each client sends the output of the local randomizer $\calR$ to a secure shuffler that randomly permutes the clients' messages before passing them to the server.}
\label{fig:setup-figure}
\end{figure}
